Multi-Decoder DPRNN: High Accuracy Source Counting and Separation

We propose an end-to-end trainable approach to single-channel speech separation with unknown number of speakers. Our approach extends the MulCat source separation backbone with additional output heads: a count-head to infer the number of speakers, and decoder-heads for reconstructing the original signals. Beyond the model, we also propose a metric on how to evaluate source separation with variable number of speakers. Specifically, we cleared up the issue on how to evaluate the quality when the ground-truth hasmore or less speakers than the ones predicted by the model. We evaluate our approach on the WSJ0-mix datasets, with mixtures up to five speakers. We demonstrate that our approach outperforms state-of-the-art in counting the number of speakers and remains competitive in quality of reconstructed signals.

==> drafts/app1.tex <==
%!TEX root = ../main.tex

\section{Approach for Variable Number of Speakers.}

{\noindent \bf Problem Formulation.}
Let $\rvx$ denote the mixed input audio, and $\gY = \{\rvy^{k}\}$ denote the set of separated audio  from each speaker. The goal is to learn a function $F(\rvx) \mapsto \gY$. It is generally challenging to handle variable number of outputs. 

To simplify the problem, we assume that $$K \geq |\gY|\;\forall (\rvx, \gY) \in \cD,$$ \ie, $K$ atleast the maximum number of speakers mixed in the dataset. In this case, we can learn a function from $F(\rvx) \mapsto \mathbb{R}^{|\rvy| \times K}$ and discard some outputs.

{\noindent \bf Background:}
Permutation Invariant Loss: 
$$\ell(\hat{\rvy}, \rvy) \triangleq \min_{i(k)} \norm{\hat{y}^{i(k)}-y^{k}} \;\; s.t. \;i(\cdot) \;\text{is a permutation}$$
As we assumed $K$ to be larger than the number of speakers, we just require:
$$\ell(\hat{\rvy}, \rvy) \triangleq \min_{i(k)} \norm{\hat{y}^{i(k)}-y^{k}} \;\; s.t. \;i(\cdot) \;\text{is an injective function}$$
\ray{One can reduce a loss to another by padding dummy $\rvy^k$s}

{\noindent \bf Idea 1:} Directly training with permutation invariant loss where we zero-pad $\gY$ up to $K$ speakers. Instead of brute-force search through all permutation, solve using Hungarian Algorithm. \ray{Issue: Need some silence detector at test time.}

{\noindent \bf Idea 2:} Attention Mechanism at the output. Let $F$ to also output $K$ attentions, $\sigma\in [0,1]^{K}$ indicating whether a predicted audio output $\hat{\rvy}^k$ should be use. 
\begin{itemize}
\item Training method 1 (end-to-end training): Apply permutation invariant loss on $\sigma \odot \hat{\rvy}$ and train end-to-end, where we zero-pad $\gY$ up to $K$ speakers. 
\item Training method 2 (joint training): Apply permutation invariant loss on $\hat{\rvy}$ based on an unbalanced assignment (we do not zero-pad here). Next, train $\sigma$ via cross-entropy loss, \ie, if assigned the label is 1 else 0.
\end{itemize}


{\noindent \bf Idea 3 (Summary from Joseph's Email):} Alternate between updating speaker vector and separated signal. Given a network $S(\rvy^k)$ that produces speaker vectors, and an extractor network $E(\rvx, S(\rvy^k))$, alternate forward passe between $S$ and $E$ until convergence. \ray{``discard channels with on/off estimation off''. That description is unclear; and discarding is obviously not differentiable."} 

==> sections/rel.tex <==
%!TEX root = ../main.tex

\section{Related Work}
{\noindent \bf Audio source separation.}
\cite{luo2019conv}
\jz{TODO}

{\noindent \bf Network architectures.}
\cite{bai2019deep}
\ray{TODO}
